Alternating Updates for Efficient Transformers

It has been well established that increasing scale in deep transformer networks leads to improved quality and performance. However, this increase in scale often comes with prohibitive increases in compute cost and inference latency. We introduce Alternating Updates (AltUp), a simple-to-implement method to increase a model's capacity without the computational burden. AltUp enables the widening of the learned representation, i.e., the token embedding, while only incurring a negligible increase in latency. AltUp achieves this by working on a subblock of the widened representation at each layer and using a predict-and-correct mechanism to update the inactivated blocks. We present extensions of AltUp, such as its applicability to the sequence dimension, and demonstrate how AltUp can be synergistically combined with existing approaches, such as Sparse Mixture-of-Experts models, to obtain efficient models with even higher capacity. Our experiments on benchmark transformer models and language tasks demonstrate the consistent effectiveness of AltUp on a diverse set of scenarios. Notably, on SuperGLUE and SQuAD benchmarks, AltUp enables up to $87\%$ speedup relative to the dense baselines at the same accuracy.

==> sec/analysis.tex <==
\section{Theoretical Arguments}
\label{sec:analysis}
In this section, we analyze and provide unifying theoretical insights into popular lookup functions (Sec.~\ref{sec:analysis-lookups}) and demonstrate the theoretical advantage of using embedding table lookups at higher layers (Sec.~\ref{sec:analysis-embedding-lookups}). 


\subsection{Lookup functions as variants of LSH and their efficiency}
\label{sec:analysis-lookups}
Here, we show that under simplifying assumptions, softmax routing and wordpiece routing can be viewed as Spherical LSH and Min-hash LSH, respectively. This interpretation will imply that, with practical configurations, Token-ID is more parameter efficient than Softmax, which is more efficient than hyperplane-LSH lookup.

{\bf Preliminaries}  We consider a Locality Sensitive Hashing (LSH) that maps an input to one of $n$ buckets. We let $r_2 > r_1 > 0$, denote the threshold for nearby points and far-away points, respectively. For $x, y \in \mathbb{R}^d$, we say $x$ and $y$ are nearby if $
\norm{x - y}_2 \leq r_1$ and they are far-away if $\norm{x - y}_2 \geq r_2$, where $\norm{x}_2$ is the $2$-norm of the vector $x$. Let $c = r_2/r_1 > 1$ denote the distance gap as a ratio. Let 
\begin{align*}
    p_1 &\le \Pr(h(x) = h(y): \norm{x - y}_2 \leq r_1)\\
    p_2 &\ge \Pr(h(x) = h(y): \norm{x - y}_2 \geq r_2)
\end{align*}
 denote lower and upper bounds on the collision probability of nearby points and far-away points, respectively. Notably, with $n$ buckets the probability that two nearby points hash to the same bucket is $n^{-\rho}$, where $\rho = \frac{\log (1/p_1)}{\log (1/p_2)}$~\cite{andoni2015optimal}. 



{\bf Efficiency} Let us consider two sentences $s_1, s_2$ of the same length $l$ that have $f$ fraction of wordpieces in common. Assume for simplicity that the embedding vector for each wordpiece is a random unit vector in $R^d$. We summarize LSH variants and the collision probability of nearby points in this setting. We are interested in the \emph{efficiency}, i.e., the collision probability for the set of experts corresponding to two similar sentences. For a fixed size table of $n$ experts, the higher the collision probability for two similar sentences, the more efficient the LSH lookup is in terms of routing similar tokens to similar buckets. The full details of the LSH variants and proofs are in the supplementary.
\begin{enumerate}
    \item \textbf{Hyperplane LSH~\cite{datar2004locality}}: this variant divides a $R^d$ space into buckets by using randomly oriented parallel equispaced hyperplanes. Hyperplane LSH has the property that $\rho = \OO(1/c)$. Computations (see supplementary) yield $c = 1/\sqrt{1- f}$, which implies a collision probability of $n^{-\OO(\sqrt{1- f})}$.
    
    %Note that lower $\rho$ value is better as it  shows up in the exponent of $n$ in the time/space complexity of nearest neighbor search \cb{If lower $\rho$ is better, doesn't that mean hyperplane LSH is better than spherical because $1 / \sqrt{1 - f^2} < 1 / (1 - f^2)$?}
    %\nishanth{I think $\rho$ is actually $\sqrt{1-f^2}$ here. that addresses $c>1$ issue also.}
    
    % Let us evaluate the probability of routing a certain token to the expert at some intermediate layer. Note that at high layers due to multiple prior attention computations, we can assume sufficient mixing has happened between the tokens. For simplicity let us think of this as averaging the value of all the token embeddings. Since the initial wordpiece embeddings are random, after averaging the dot product between the two averages will be $f$ and so the distance between them will be $\sqrt{1- f^2}$. Instead if we take two sentences with no tokens in common the distance between them will be $O(1)$. This gives a $c = 1/\sqrt{1- f^2}$ and $\rho = \OO(\sqrt{1- f^2})$. With $n$ experts this will give a collision probability of $n^{-\OO(\sqrt{1- f^2})}$ for the set of experts corresponding to the two similar sentences.
    
    \item \textbf{Spherical LSH \cite{andoni2008near}}: here, we use a random set of points to divide up the $R^d$ space into Voronoi regions, each representing a different bucket. This method has a better $\rho$ value of $\OO(1/c^2)$. Assuming that the Softmax lookup matrix $W$ (see Sec.~\ref{sec:routing-functions}) is uniform, the Softmax lookup corresponds to Spherical LSH~\cite{andoni2015practical}. This yields $\rho = \OO(1- f)$ and a collision probability of $n^{-\OO(1- f)}$.
    
    \item \textbf{Min-hash~\cite{broder1998min}}: this approach is used for hashing sets so that similar sets get hashed to the same bucket. Using the Jaccard similarity measure for comparing sets means that the fraction of experts that match up for the two sentences $s_1,s_2$ is $f$. This also means that Token-ID lookup can be viewed as Min-hash LSH.
    
    %(for two sets $A,B$ it is given by $sim(A,B) = |A \cap B|/|A \cup B|$) then this hash function ensures that two sets $A,B$ will hash to the same bucket with probability equal to $sim(A,B)$.
    
    %This is done by hashing the universe of elements from which the sets are constructed randomly into some interval in the real line, and hashing a set to the element that has the smallest value on the real line. Thus each element can be viewed as a bucket. If we use the Jaccard similarity measure  for comparing sets (for two sets $A,B$ it is given by $sim(A,B) = |A \cap B|/|A \cup B|$) then this hash function ensures that two sets $A,B$ will hash to the same bucket with probability equal to $sim(A,B)$. Note that this same property holds for wordpiece based routing as each token at any layer is hashed to an expert specific to that wordpiece. Thus the fraction of experts that match up for the two sentences $s_1,s_2$ is $f$. In this sense wordpiece based routing is similar to min-hash LSH.
\end{enumerate}



The above properties imply the following theorem.
%\cb{Does most efficient mean lowest collision probability? highest-Rina}
% \begin{theorem}
% \label{thm:lookup-efficiency}
% In the setting of the above simplifying assumptions, we have the following:
% \begin{enumerate}
%     \item Softmax and Token-ID lookup can be viewed as Spherical LSH and Min-hash LSH, respectively.
%     \item The probability that a random token in the two sentences of equal length that overlap in $f$ fraction of the wordpieces gets routed to the same expert is $n^{-\OO\left(\sqrt{1- f^2}\right)}$, $n^{-\OO\left(1- f^2\right)}$, and $f$ for hyperplane LSH, Softmax, and Token-ID lookup, respectively.
%     \item For large $n$ and a small fraction $f$, in terms of routing to the same expert, the efficacy order of the different lookup methods is $\text{Token-ID} \ge \text{Softmax} \ge \text{hyperlane LSH}$. 
%     %\cb{Is this saying that $f \leq n^{-O(1/(1- f^2))} \leq n^{-O\left(1/\sqrt{1- f^2}\right)}$? Fixed: Rina}
% \end{enumerate}
% \end{theorem}

\begin{restatable}{theorem}{lookupefficiency}
\label{thm:lookup-efficiency}
In the setting of the above simplifying assumptions, we have the following:
\begin{enumerate}
    \item Softmax and Token-ID lookup can be viewed as Spherical LSH and Min-hash LSH, respectively.
    \item The probability that a random token in the two sentences of equal length that overlap in $f$ fraction of the wordpieces gets routed to the same expert is $n^{-\OO\left(\sqrt{1- f}\right)}$, $n^{-\OO\left(1- f\right)}$, and $f$ for hyperplane LSH, Softmax, and Token-ID lookup, respectively.
    \item For large $n$ and a small fraction $f$, in terms of routing to the same expert, the efficacy order of the different lookup methods is $\text{Token-ID} \ge \text{Softmax} \ge \text{hyperlane LSH}$. 
    %\cb{Is this saying that $f \leq n^{-O(1/(1- f^2))} \leq n^{-O\left(1/\sqrt{1- f^2}\right)}$? Fixed: Rina}
\end{enumerate}
\end{restatable}


% \begin{theorem}
% In the setting of the above simplifying assumptions, the following holds:
% routing based on softmax and wordpiece can be viewed as Spherical LSH and and Min-hash LSH, respectively.
% The probability that a random token in the two sentences of equal length that overlap in $f$ fraction of the wordpieces gets routed to the same expert is $n^{-O\left(1/\sqrt{1- f^2}\right)}$, $n^{-O(1/(1- f^2))}$, and $f$ for Hyperplane LSH routing, softmax routing, and wordpiece routing, respectively. For large $n$ and a small fraction $f$, this shows that in terms of routing to same expert, the efficacy order of the different routing methods is $\text{wordpiece-routing} \ge \text{softmax-routing} \ge \text{hyperlane-LSH-routing}$. \cb{Is this saying that $f \leq n^{-O(1/(1- f^2))} \leq n^{-O\left(1/\sqrt{1- f^2}\right)}$?}
% \end{theorem}

% \begin{theorem}
% Softmax routing with a random softmax layer can be viewed as spherical LSH
% wordpiece routing can be viewed as Min-hash based LSH which is theoretically known to be a better LSH than spherical LSH or hyperplane LSH
% \end{theorem}

\subsection{Advantage of embedding lookups at higher layers}
\label{sec:analysis-embedding-lookups}

Note that the Token-ID routing need not be a per-layer routing operation since it is merely a function of the token ID which can be done once in the input layer. One way of incorporating the result of this lookup is to simply feed the output of the lookup into the input for the first layer. This implementation delegates the work of passing on this information to the higher layers to the network itself. Alternatively, the output of the lookup in the input layer can be partitioned so that \emph{different parts of the lookup output feed into the different layers of the network}. This partitioning and feeding the embedding lookup directly to the layers can be viewed as separate embedding lookups in those layers. 

The theorem below establishes that the latter implementation with embedding lookups at higher layers enables a more efficient architecture of lower width and fewer parameters than the former one.

%Note that in Token-ID routing (see Sec.~\ref{sec:routing-functions}), although conceptually it involves a lookup at each layer, all these lookups can be combined in to a single "embedding lookup" that can be done at the input layer. Normally embedding lookups are done on categorical features at input layer and fed directly into the next layer. In the wordpiece routing scenario different parts of the lookup output feed into different layers resulting in a different architecture.




\begin{restatable}{theorem}{embeddinglookup}
\label{thm:embedding-lookup}
There exists a class of natural learning problems where embedding lookups of categorical features at upper layers in addition to the input layer gives a more efficient architecture compared to an architecture that feeds the embedding lookup output only to the input layer.
\end{restatable}
\begin{proof}[Proof Sketch]
The main idea is to consider two architectures that implement the embedding lookup in the two distinct ways and an input $(u, q)$ with ground truth score $\dotp{\Psi(u)}{\Phi(q)}$, where $\Psi(u)$ maps $u$ to a $d$-dimensional feature vector and $\Phi(q)$ is a non-linear transformation of $q$ that can be implemented by a deep network of width $d$. The first architecture combines the lookup $\Psi(u)$ with $q$ (by a weighted sum) and feeds into the network as input; the second architecture in addition feeds the embedding output of $u$ to all the layers of the network instead of only the lowest layer. The second architecture can store $\Psi(u)$ in the table and feed it directly to the output layer (which produces $\Phi(q)$) to obtain the result $\dotp{\Psi(u)}{\Phi(q)}$ using width $d$. On the other hand, for the first architecture the entropy of the information carried up the layers is at least $2d$ assuming $u$ and $q$ are random and not correlated, and so the width of the network needs to be $2d$.

% \cb{Original proof below} 

% % Original version
% Consider a scenario where one is scoring between pair of (url, query-feature)  where the url comes a single categorical feature $u$ and a query feature vector $\vec q$. Assume that the ground truth score is given by a dot product $\dotp{\Psi(u)}{\Phi(q)}$ where $\Psi$ produces a url feature vector for the given url $u$ and $\Phi$ is a non-linear transform on the query vector q. Assume $\Psi(u)$, $q$, and $\Phi(q)$ are $d$ dimensional and the operation $\Phi$ can be implemented by a deep network of a certain depth (say $h$).

% Now consider two architectures both of which convert the url into a $d$ dim feature vector based on an embedding lookup: The first architecture combines the lookup url feature vector with $q$ (by a weighted sum) and feeds into a depth $h$ network; the second architecture in addition feeds the embedding output of $u$ to all the layers of the network instead of only the lowest layer. We will show that in the former case the depth of the network needs to be $2d$ and in the latter case only $d$ to represent the ground truth function. In the latter case the ground truth can be represented by storing $\Psi(u)$ in the embedding table entry for $u$ and the network. By using the weighted sum that gives weight $0$ to the url feature and $1$ to the query features, we can have a network of width $d$ and height $h$ that implements $\Phi$. However in the former case since $\Phi(u)$ is not available at the output layer, it needs to be carried up the network along with the processing of the query features $q$. Assuming $q$ and $u$ inputs are random and not correlated, the entropy of the information carried up the layers is at least $2d$ and so the width of the network needs to be at least $2d$.
\end{proof}

==> sec/limitations.tex <==
\section{Limitations and future work}
\label{sec:limitations}
\cb{TODO: Limitations}

==> sec/routing.tex <==
\section{Lookup Functions}
\label{sec:routing-functions}

In this section, we formalize the augmentation of a layer $L$ with external memory and provide an overview of the various lookup functions that we cover in this paper. The memory augmented layer is shown as Alg.~\ref{alg:mal}. Since we are primarily interested in Transformer-like architectures we can just focus on the action of the layer on a single token. Abstractly, we consider a layer $L$ to be a function from a vector space $\cX$ to itself. For example, $L$ can be the self-attention layer of a transformer and $\cX$ the space of embedded token vectors $\R^{\embdim}$. We let $\functions$ be the set of all functions from $\cX$ to $\cX$. The external memory for the layer consists of a lookup function $\lookup$ and a memory table $\memtable$. 


Given the previous layer output $x \in \cX$ and the index of original token in the vocabulary (i.e.\ the token-id, see Sec.~\ref{sec:token-id-routing}) which we denote $\id$, the look-up function $\lookup$ computes a set of indices $\experts = \lookup(x, \id)$. Typically the look-up function either uses only $\id$ as in Token-ID lookup (see Sec.~\ref{sec:token-id-routing}) or only $x$ as in Softmax lookup (see Sec.~\ref{sec:softmax-routing}). The indices $i \in \experts$ are then used to access the table $\memtable$ and access experts $f_i = \memtable(i)$ in $\functions$. 

We will consider experts $f_i$ that are either two-layer fully connected networks $f(x) = V\phi(U^Tx)$ where $\phi$ is the ReLU activation or just simply a constant function $f(x) = b$. For a $d$-dimensional input, the matrices $V,U \in \mathbb{R}^{d \times \mathrm{rank}}$, where  $\mathrm{rank}$ is a configurable parameter that specifies the width of the expert, and consequently the computation time of routing to each partial expert. The augmented layer computation outputs $L(x) + \sum_{i \in \experts} w_i(x) f_i(x)$ for some weighting functions $w_i$ instead of the normal output $L(x)$. In principle, one could consider alternate ways of combing $L(x)$ and $\sum_{i} w_i(x) f_i(x)$, however in this work we only consider addition since it is simple and preserves dimensions. We consider different choices of the lookup function $\lookup$ and memory tables $\memtable$ as follows.
\begin{algorithm}
\label{alg:augment-memory}
%\SetAlgoLined
\begin{algorithmic}[1]
\INPUT{Layer $L \in \functions$, previous layer output $x \in \cX$, $\id \in \N$, look-up function $\lookup : \cX \times \N \to [\tablesize]$, memory table $\memtable : [\tablesize] \to \functions$
}
\STATE Table index $i = \lookup(x, \id)$\;
\STATE Adjustment function $f = \memtable(i)$\;
\OUTPUT{$L(x) + f(x)$}
\end{algorithmic}
\caption{Memory Augmented Layer}\label{alg:mal}
\end{algorithm}

\subsection{MoE-style Softmax Lookup}\label{sec:softmax-routing}
The MoE layer routes an input token $x$ to $k$ of $n$ experts where each expert is itself a parametrized subnetwork (e.g., a fully-connected layer). Following~\cite{fedus2022review}, we let $\{E_i(\cdot)\}_{i \in [n]}$ and $E_i(x)$ denote the set of experts and the output of lookup the input token $x$ to expert $i$, respectively. For an input token $x$, a learnable weight matrix $W$ is applied to obtain the logits $h(x) = W x$. The lookup probabilities are computed by taking the softmax of $h(x)$
$$
p_i(x) = \frac{\exp(h_i(x))}{\sum_{j \in [n]} \exp(h_j(x))} \quad \forall{i \in [n]}.
$$
The token $x$ is routed to the expert(s) $\TT \subset [n]$ with the top-$k$ probabilities $p(x)$. Since this operation is not differentiable, the output $y$ is computed as a probability weighted combination of the experts' outputs to enable gradients to propagate back to the router parameters, i.e.,
$
y = \sum_{i \in \TT} p_i(x) E_i(x)
$
~\cite{shazeer2017outrageously}.

\subsection{Token-ID Lookup}\label{sec:token-id-routing}
In a transformer, the computation can be viewed as repeatedly transforming the embedding vector of a token within the initial embedding space. For example the token ``tiger" may be embedded initially as $x_0 \in \R^{\embdim}$ and then transformed into $x_1, x_2, \ldots$, etc.\ successively where each $x_i \in \R^{\embdim}$. In Token-ID lookup for each $x_i$ the look-up function $\lookup$ (see Alg.~\ref{alg:mal}) simply returns the index of the input token (e.g.\ ``tiger") in the vocabulary and ignores the previous layer output. Note that in this case the table size $\tablesize$ of each layer is equal to the size of the vocabulary.


\subsection{Locality Sensitive Hashing (LSH) Lookup}
Locality Sensitive Hashing~\cite{gionis1999similarity} is a popular variant of hashing that tends to hash similar objects to the same buckets and is used for approximate nearest neighbor search~\cite{andoni2014beyond, andoni2015optimal, andoni2015practical}. It tends to hash similar inputs to the same bucket with higher probability and dissimilar inputs to different buckets. There are variants of LSH, but for LSH lookup we follow prior work~\cite{baykal2022theoretical,panigrahy2021sketch} and consider the \emph{hyperplane-based LSH}. At a high level, this approach partitions the input space into a grid-like structure using randomly oriented, equispaced hyperplanes. Each such region is considered a bucket (expert) of the hash table. See Sec.~\ref{sec:analysis} and the supplementary material for details.



% \section{Theoretical Arguments}

% \subsection{Viewing different routing/lookup methods as type of locality sensitive hash functions}

% \cb{Maybe move some of the content to the previous section on routing functions?}
% {\bf Locality Sensitive Hashing}  Let us look at an LSH that maps an input to one (or a few locations) out of the  $m$ hash buckets. It is well-known that LSH provably provides sub-linear query time and sub-quadratic space complexity for approximate nearest neighbor search. More specifically, fix $0 < r_1 < r_2$, where $r_1$ is the threshold for nearby points, and $r_2$ is the threshold for far-away points, i.e. for $x, y \in \mathbb{R}^d$, we say $x$ and $y$ are nearby if $|x - y|_2 \leq r_1$ and they are far-away if $|x - y|_2 \geq r_2$, where $|x|_2$ is the $2$-norm of the vector $x$. Let $c = r_2/r_1 > 0$ denote the distance gap as a ratio. Let $p_1 \le Pr(h(x) = h(y): |x - y|_2 \leq r_1)$ and $p_2 \ge Pr(h(x) = h(y): |x - y|_2 \geq r_2)$ denote lower and upper bounds on the collision probability of nearby points and far-away points, respectively. Define $\rho = \frac{\log (1/p_1)}{\log (1/p_2)}$. Then LSH-based nearest neighbor search has a $O(n^{\rho})$  query time and $O(n^{1 + \rho})$ space complexity for a $c$ approximate nearest neighbor query~\cite{andoni2014beyond, andoni2015optimal, andoni2015practical}. With $n$ buckets the probability that two nearby points hash to the same bucket is $n^{-\rho}$.

% \cb{Need to shorten this section/put it in the appendix}
% There are different variants of LSH and we will see how they correspond to different types of routing functions. Let us consider two sentences $s_1, s_2$ of the same length $l$ that have $f$ fraction of wordpieces in common. Assume for simplicity that the embedding vector for each wordpiece is a random vector in $R^d$. 

% 1. Hyperplane based LSH \cite{datar2004locality}: This method divides a $R^d$ space by using randomly oriented parallel equispaced hyperplanes. By using a few such such random orientations and taking the intersections of the regions divides the space into a lattice/grid like structure of higher dimensional parallelopipeds. Each such region is considered to be one hash bucket (by further hashing regions to experts one can interpret this as an expert routing algorithm). It is known that by choosing the the gap between consecutive parallel hyperplanes in a specific way one can get a $\rho$ value of $O(1/c)$; Note that lower the $\rho$ value better is the LSH as it shows up in the exponent of $n$ in the time/space complexity of nearest neighbor search. 

% Let is evaluate the probability of routing a certain token to the expert at some high layer. Note that at high layers due to attention sufficient mixing has happened between the tokens. For simplicity let us think of this as averaging the value of all the token embeddings. Since the initial wordpiece embeddings are random, after averaging the dot product between the the two averages will be $f$ and so the distance between them will be $\sqrt{1- f^2}$. Instead if we take two sentences with no tokens in common the distance between them will be $O(1)$. This gives a $c = \sqrt{1- f^2}$ and $\rho = O(1/\sqrt{1- f^2})$. With $n$ experts this will give a collision probability of $n^{-O(1/\sqrt{1- f^2})}$ for the set of experts corresponding to the two similar sentences.

% 2. Spherical LSH \cite{andoni2008near}: This method instead of using hyperplanes, uses a random set of points and divides up the $R^d$ space into the voronoi regions formed by these points and each voronoi cell is one hash bucket. This method has a better $\rho$ value of $O(1/c^2)$. Note that the softmax based routing where the softmax matrix is random corresponds to this LSH -- if we take all rows in the matrix as unit norm, then the dot product will with the top-1 routing will correspond to picking the expert whose routing vector is closest in angle to the input vector (this is studied in \cite{andoni2015practical}). 

% Based on the previous analysis this gives $\rho = O(1/(1- f^2))$. This will give a collision probability of $n^{-O(1/(1- f^2))}$ for the set of experts corresponding to the two similar sentences.

% 3. Min Hashing for set similarity \cite{broder1998min}: This is a method for hashing a set so that similar sets get hashed to the same bucket. This is done by hashing the universe of elements from which the sets are constructed randomly into some interval in the real line, and hashing a set to the element that has the smallest value on the real line. Thus each element can be viewed as a bucket. If we use the Jaccard simlarity measure  for comparing sets (for two sets $A,B$ it is given by $sim(A,B) = |A \cap B|/|A \cup B|$) then this hash function ensures that two sets $A,B$ will hash to the same bucket with probability equal to $sim(A,B)$.

% Note that this same property holds for wordpiece based routing as each token at any layer is hashed to an expert specific to that wordpiece. Thus the fraction of experts that match up for the two sentences $s_1,s_2$ is $f$. In this sense wordpiece based routing is similar to min hash based LSH. This gives

% \begin{theorem}
% Under above  simplifying assumptions routing based on hyperplane-LSH, softmax, and wordpiece can be viewed as hyperplane-LSH, spherical-LSH, and min-hash LSH respectively.
% The probability that a random token in the two sentences of equal length that overlap in $f$ fraction of the wordpieces gets routed to the same expert is $n^{-O\left(1/\sqrt{1- f^2}\right)}$, $n^{-O(1/(1- f^2))}$, and $f$ respectively. For large $n$ and a small fraction $f$, this shows that in terms of routing to same expert, the efficacy order of the different routing methods is $\text{wordpiece-routing} > \text{softmax-routing} > \text{hyperlane-LSH-routing}$.
% \end{theorem}

% % \begin{theorem}
% % Softmax routing with a random softmax layer can be viewed as spherical LSH
% % wordpiece routing can be viewed as Min-hash based LSH which is theoretically known to be a better LSH than spherical LSH or hyperplane LSH
% % \end{theorem}

% \subsection{Advantage of Embedding lookups at higher layers}

% Note that in wordpiece based routing, although conceptually it involves a lookup at each layer, all these lookups can be combined in to a single "embedding lookup" that can be done at the input layer. Normally embedding lookups are done on categorical features at input layer and fed directly into the next layer. In the wordpiece routing scenario different parts of the lookup output feed into different layers resulting in a different architecture. We will now argue that this an result in a more efficient architecture of lower width and fewer parameters.

% \cb{We can move this to the appendix as the proof}
% Consider a scenario where one is scoring between pair of <url, query-feature>  where the url comes a single categorical feature $u$ and a query feature vector $\vec q$. Assume that the ground truth score is given by a dot product $<\Psi(u). \Phi(q)>$ where $\Psi$ produces a url feature vector for the given url $u$ and $\Phi$ is a non-linear transform on the query vector q. Assume both $\Psi(u)$, $q$, and $\Phi(q)$ are $d$ dimensional and the operation $\Phi$ can be implemented by a deep network of a certain depth (say $h$).

% Now consider two architectures both of which convert the url into a $d$ dim feature vector based on an embedding lookup: The first architecture combines the lookup url feature vector with $q$ (by a weighted sum) and feeds into a depth $h$ network; the second architecture in addition feeds the embedding output of $u$ to all the layers of the network instead of only the lowest layer. We will show that in the former case the depth of the network needs to be $2d$ and in the latter case only $d$ to represent the ground truth function. In the latter case the ground truth can be represented by storing $\Psi(u)$ in the embedding table entry for $u$ and the network. By using the weighted sum that gives weight $0$ to the url feature and $1$ to the query features, we can have a network of width $d$ and height $h$ that implements $\Phi$. However in the former case since $\Phi(u)$ is not available at the output layer, it needs to be carried up the network along with the processing of the query features $q$. Assuming $q$ and $u$ inputs are random and not correlated, the entropy of the information carried up the layers is at least $2d$ and so the width of the network needs to be at least $2d$. This proves:

% \begin{theorem}
% There exist learning problems where embedding lookups of categorical features at upper layers in addition to the input layer gives a more efficient architecture compared to an architecture that feeds embedding lookup only to the input layer.
% \end{theorem}

% \begin{theorem}
% Although wordpiece based lookup can be combined into a single embedding lookup, there may be scenarious where attaching and consuming different copies of the embedding table at different layers is better than a single embedding table at the input layer.
% \end{theorem}


==> sec/softmax.tex <==
\section{MoE-style Routing}
\label{sec:softmax}
The MoE layer routes an input token $x$ to $k$ of $n$ experts where each expert is a subset of network parameters (e.g., a fully-connected layer). Following~\cite{fedus2022review}, we let $\{E_i(\cdot)\}_{i \in [N]}$ and $E_i(x)$ denote the set of experts and the output of routing the input token $x$ to expert $i$, respectively. For an input token $x$, a learnable weight matrix $W$ is applied to obtain the logits $h(x) = W x$. The routing probabilities are computed by taking the softmax of $h(x)$
$$
p_i(x) = \frac{\exp(h_i(x))}{\sum_{j \in [N]} \exp(h_j(x))} \quad \forall{i \in [n]}.
$$
The token $x$ is routed to the expert(s) $\TT \subset [n]$ with the top-$k$ probabilities $p(x)$. Since this operation is not differentiable, the output $y$ is computed as a probability weighted combination of the experts' outputs to enable gradients to propagate back to the router parameters, i.e.,
$
y = \sum_{i \in \TT} p_i(x) E_i(x).
$


